A type system for data flow and alias analysis in ReScript

ReScript introduces a strongly typed language that targets JavaScript, as an alternative to gradually typed languages, such as TypeScript. In this paper, we present a type system for data-flow analysis for a subset of the ReScript language, more specific for a lambda-calculus with mutability and pattern matching. The type system is a local analysis that collects information about what variables are used and alias information.

==> examples/DFAbs.tex <==
\begin{figure}
\begin{tabular}{l}
App-1:\\
\inference[\runa{App}]
{
	\inference[\runa{Var}]{}
	{env'\vdash \left\langle x^3,sto,\psi_1,2\right\rangle\rightarrow\left\langle v,sto,\psi_1,(\emptyset,\{x^3\}),3 \right\rangle}
	\;\;
	\inference[\runa{Cons}]{}
	{env'\vdash \left\langle 1^4,sto,\psi_1,3\right\rangle\rightarrow\left\langle 1,sto,\psi_1,(\emptyset,\emptyset),4 \right\rangle}
	\\
	\inference[\runa{Var}]{}
	{env[y\mapsto 1]\vdash \left\langle y^1,sto,\psi_2,4\right\rangle\rightarrow\left\langle 1,sto,\psi_2,(\emptyset,\{y^1\}),1 \right\rangle}
}
{env'\vdash \left\langle[x^3\;1^4]^5,sto,\psi_1,2\right\rangle\rightarrow\left\langle 1,sto,\psi_2,(\emptyset,\{y^1,x^3\}),5 \right\rangle}\\
Where $env'(x)=v=\left\langle y,y^1,env \right\rangle$, $inf_{\psi_1}(x)=2$, $\;\psi_1=(w_1,\sqsubseteq_w^1)$, $w_1(x^2)=(\emptyset,\emptyset)$, $inf_{\psi_1}(y)=\epsilon$, $w_2=w_1[y^4\mapsto(\emptyset,\emptyset)]$, $\psi_2=(w_2,\sqsubseteq_w^1)$,\\
$inf_{\psi_2}(y)=4$, and $w_2(y^4)=(\emptyset,\emptyset)$\\[0.5cm]

App-2:\\
\inference[\runa{App}]
{
	\inference[\runa{Var}]{}
	{env''\vdash \left\langle x^6,sto,\psi_2,2\right\rangle\rightarrow\left\langle v,sto,\psi_2,(\emptyset,\{x^6\}),6 \right\rangle}
	\;\;
	\inference[\runa{Cons}]{}
	{env''\vdash \left\langle 2^7,sto,\psi_2,6\right\rangle\rightarrow\left\langle 2,sto,\psi_2,(\emptyset,\emptyset),7 \right\rangle}
	\\
	\inference[\runa{Var}]{}
	{env[y\mapsto 2]\vdash \left\langle y^1,sto,\psi',7\right\rangle\rightarrow\left\langle 1,sto,\psi',(\emptyset,\{y^1\}),1\right\rangle}
}
{env''\vdash \left\langle[x^6\;2^7]^8,sto,\psi_2,5\right\rangle\rightarrow\left\langle 2,sto,\psi',(\emptyset,\{y^1,x^6\}),8 \right\rangle}\\
Where $env'(x)=v=\left\langle y,y^1,env \right\rangle$, $inf_{\psi_2}(x)=2$, $\;\psi_2=(w_2,\sqsubseteq_w^2)$, $w_2(x^2)=(\emptyset,\emptyset)$, $inf_{\psi_2}(y)=4$, $w_3=w_2[y^7\mapsto(\emptyset,\emptyset)]$, $\psi'=(w_3,\sqsubseteq_w^2\cup(4,7))$,\\
$inf_{\psi'}(y)=7$, and $w_3(y^7)=(\emptyset,\emptyset)$\\[0.5cm]

Let-1:\\
\inference[\runa{Let}]
{
	\inference[App-1]{}
	{env'\vdash \left\langle[x^3\;1^4]^5,sto,\psi_1,2\right\rangle\rightarrow\left\langle 1,sto,\psi_2,(\emptyset,\{y^1,x^3\}),5 \right\rangle}
	\;\;
	\inference[App-2:]{}
	{env''\vdash \left\langle[x^6\;2^7]^8,sto,\psi_2,5\right\rangle\rightarrow\left\langle 2,sto,\psi',(\emptyset,\{y^1,x^6\}),8 \right\rangle}
}
{env'\vdash \left\langle[let\;z\;(x^3\;1^4)^5\;(x^6\;2^7)^{8}]^{9},sto,\psi_1,2\right\rangle\rightarrow\left\langle 2,sto,\psi',(\emptyset,\{y^1,x^6\}),9 \right\rangle}\\
Where $env''=env[z\mapsto 1]$, $\psi_1=(w_1,\sqsubseteq_w^1)$, and $\psi_2=(w_1[z^{5}\mapsto(\emptyset,\emptyset)],\sqsubseteq_w^1)$\\[0.5cm]

\inference[\runa{Let}]
{
	\inference[\runa{Abs}]
	{}
	{env\vdash \left\langle[\lambda\; y.(y^1)]^2,sto,\psi,0\right\rangle\rightarrow\left\langle v,sto,\psi,(\emptyset,\emptyset),2 \right\rangle}
	\;\;
	\inference[Let-1:]{}
	{env'\vdash \left\langle[let\;z\;(x^3\;1^4)^5\;(x^6\;2^7)^{8}]^{9},sto,\psi_1,2\right\rangle\rightarrow\left\langle 2,sto,\psi',(\emptyset,\{y^1,x^6\}),9 \right\rangle}
}
{env\vdash \left\langle[(let\;x\;(\lambda\;y.(y^1))^2\;(let\;z\;(x^3\;1^4)^5\;(x^6\;2^7)^{8})^{9})]^{10},sto,\psi,0\right\rangle\rightarrow\left\langle 2,sto,\psi',(\emptyset,\{y^1,x^6\}),10 \right\rangle}\\
Where $v=\left\langle y,y^1,env \right\rangle$, $env'=env[x\mapsto v]$, $\psi=(w,\sqsubseteq_w)$, and $\psi_1=(w[x^{2}\mapsto(\emptyset,\emptyset)],\sqsubseteq_w)$\\
\end{tabular}
\caption{Abstraction example}\label{FigEx.Abs}
\end{figure}



==> examples/absFig/1.tex <==
	\begin{tabular}{l}
		\inference[$APP$]
		{
			\inference[$ABS$]
			{
				\inference[$APP$]
				{
					\inference[$VAR$]{}{\Gamma';\Pi\vdash x^{p}:\alpha:T'\rightarrow T''}
					\;\;\;
					\inference[$VAR$]{}{\Gamma';\Pi\vdash z^{p'}:(\{z^{p'}\},\emptyset)}
				}
				{\Gamma,x:T_1;\Pi\vdash [x^{p}\;z^{p'}]^{p''}:T''\{\alpha / (\{z^{p'}\},\emptyset)\}}
			}
			{\Gamma;\Pi\vdash [\lambda\; x.([x^{p}\;z^{p'}]^{p''})]^{p_3}:x:T_1\rightarrow T''\{\alpha / (\{z^{p'}\},\emptyset)\}}
			\;\;
			\inference[$ABS$]
			{
					\inference[$VAR$]{}{\Gamma,y:T;\Pi\vdash y^{p_3}:T}
			}
			{\Gamma';\Pi\vdash \lambda y.[y^{p_3}]^{p_4})]^{p_5}:y:T\rightarrow T}
		}
		{\Gamma;\Pi\vdash [[\lambda x.[x^{p}\;z^{p'}]^{p''}]^{p_3}\;[\lambda y.y^{p_4}]^{p_5}]^{p_6}:T''\{\alpha / (\{z^{p'}\},\emptyset)\}\{x / T\rightarrow T\}}\\
		Where $T_1=\alpha:T'\rightarrow T''$
	\end{tabular}


==> examples/absFig/2.tex <==
	\begin{tabular}{l}
		\inference[$APP$]
		{
			\inference[$ABS$]
			{
				\inference[$APP$]
				{
					\inference[$VAR$]{}{\Gamma';\Upsilon;\Pi\vdash x^{p}:\alpha:T\rightarrow T}
					\;\;\;
					\inference[$VAR$]{}{\Gamma';\Upsilon;\Pi\vdash z^{p'}:(\{z^{p'}\},\emptyset)}
				}
				{\Gamma,x:T\rightarrow T;\Upsilon;\Pi\vdash [x^{p}\;z^{p'}]^{p''}:T\{\alpha / (\{z^{p'}\},\emptyset)\}}
			}
			{\Gamma;\Upsilon;\Pi\vdash [\lambda\; x.([x^{p}\;z^{p'}]^{p''})]^{p_3}:x:(T\rightarrow T)\rightarrow T\{\alpha / (\{z^{p'}\},\emptyset)\}}
			\;\;
			\inference[$ABS$]
			{
					\inference[$VAR$]{}{\Gamma,y:T;\Upsilon;\Pi\vdash y^{p_3}:T}
			}
			{\Gamma';\Upsilon;\Pi\vdash \lambda y.[y^{p_3}]^{p_4})]^{p_5}:y:T\rightarrow T}
		}
		{\Gamma;\Upsilon;\Pi\vdash [[\lambda x.[x^{p}\;z^{p'}]^{p''}]^{p_3}\;[\lambda y.y^{p_4}]^{p_5}]^{p_6}:T\{\alpha / (\{z^{p'}\},\emptyset)\}\{x / T\rightarrow T\}}\\
	\end{tabular}


==> examples/absFig/3.tex <==
	\begin{tabular}{l}
		\inference[$APP$]
		{
			\inference[$ABS$]
			{
				\inference[$APP$]
				{
					\inference[$VAR$]{}{\Gamma';\Upsilon;\Pi\vdash x^{p}:\alpha:T\rightarrow T}
					\;\;\;
					\inference[$VAR$]{}{\Gamma';\Upsilon;\Pi\vdash z^{p'}:(\{z^{p'}\},\emptyset)}
				}
				{\Gamma,x:T\rightarrow T;\Upsilon;\Pi\vdash [x^{p}\;z^{p'}]^{p''}:T\{\alpha / (\{z^{p'}\},\emptyset)\}}
			}
			{\Gamma;\Upsilon;\Pi\vdash [\lambda\; x.([x^{p}\;z^{p'}]^{p''})]^{p_3}:x:(T\rightarrow T)\rightarrow T\{\alpha / (\{z^{p'}\},\emptyset)\}}
			\;\;
			\inference[$ABS$]
			{
					\inference[$VAR$]{}{\Gamma,y:T;\Upsilon;\Pi\vdash y^{p_3}:T}
			}
			{\Gamma';\Upsilon;\Pi\vdash \lambda y.[y^{p_3}]^{p_4})]^{p_5}:y:T\rightarrow T}
		}
		{\Gamma;\Upsilon;\Pi\vdash [[\lambda x.[x^{p}\;z^{p'}]^{p''}]^{p_3}\;[\lambda y.y^{p_4}]^{p_5}]^{p_6}:(\{z^{p'}\},\emptyset)}\\
	\end{tabular}


==> examples/caseFig/case.tex <==
\begin{tabular}{l}
	\inference[$CASE$]
	{
		\inference[$Cons$]{}{\Gamma;\Pi\vdash 1:(\emptyset,\emptyset) }
		\;\;
		\inference[$Pattern$]
		{
			\inference[$Var$]{} {\Gamma;\Pi\vdash x:(\{x\},\{\nu x\})}
		}
		{\Gamma;\Pi\vdash [1\;(x)]:(\{x\},\{\nu x\}) }
		\;\;
		$Case_1$
		\;\;
		$Case_2$
	}
{\Gamma;\Pi\vdash [case\;(1)\;\{(1\;(x))\;(2\;(y))\;(3\;(ref\;(1)))\}]:(\{x,y\},\{\nu x, \nu y, \nu z\})}\\
\end{tabular}



==> examples/caseFig/case1.tex <==
\begin{tabular}{l}
		\inference[$Pattern$]
		{
			\inference[$Var$]{} {\Gamma;\Pi\vdash y:(\{y\},\{\nu y\})}
		}
		{\Gamma;\Pi\vdash [2\;(y)]:(\{y\},\{\nu y\}) }
\end{tabular}


==> examples/caseFig/case2.tex <==
\begin{tabular}{l}
		\inference[$Pattern$]
		{
			\inference[$Ref$]
			{
				\inference[$Cons$]{}{\Gamma;\Pi\vdash 10:(\emptyset,\emptyset) }
			}
			{\Gamma,\nu z:(\emptyset,\emptyset);\Pi\vdash [ref\;(10)]:(\emptyset,\{\nu z\})}
		}
		{\Gamma;\Pi\vdash [3\;(ref\;(1))]:(\emptyset,\{\nu z\})}
\end{tabular}


==> examples/caseFig/letCase1.tex <==
\begin{tabular}{l}
	\inference[$let$]
	{
		\inference[$Case$]{}
		{\Gamma;\Pi\vdash [caseEx]:T}
		\;\;
		\inference[$Ref\;read$]
		{
			\inference[$Var$]{}{\Gamma;\Pi\vdash z:T\cup(\{z\},\emptyset)}
		}
		{\Gamma,z:T;\Pi\vdash [!z]:T'}
	}
{\Gamma;\Pi\vdash [\mbox{let}\;z\;(caseEx)\;(!z)]:T'}\\
Where $T'=(\{x,y,z,\nu x,\nu y,\nu z\},\emptyset)$
\end{tabular}



==> examples/caseFig/letCase2.tex <==
\begin{tabular}{l}
	\inference[$let$]
	{
		\inference[$Case$]{}
		{\Gamma;\Pi\vdash [caseEx]:T}
		\;\;
		\inference[$Ref\;read$]
		{
			\inference[$Var$]{}{\Gamma;\Pi\vdash x:(\{x\},\{\nu x\})}
		}
		{\Gamma,z:T;\Pi\vdash [!x]:T'}
	}
{\Gamma;\Pi\vdash [\mbox{let}\;z\;(caseEx)\;(!x)]:T'}\\
Where $T'=(\{x,\nu x\},\emptyset)$
\end{tabular}



==> sections/Proof/TProof/cons.tex <==
\item[\runa{Cons}] Here, $e^p=c^p$, where we have:
			\begin{itemize}
				\item $\Gamma,\Pi\vdash c^p :(\emptyset,\emptyset)$,
				\item $env\vdash\left\langle c^p,w,sto,p'\right\rangle\rightarrow\left\langle c,w,sto,(\emptyset,\emptyset),p\right\rangle$
			\end{itemize}
			and that $(w,env)\models\Gamma$ and $(w,env)\models(\emptyset,\emptyset)$.

			This case follows immediately, since we can conclude that $\Gamma,\Pi\vdash c:(\emptyset,\emptyset)$, because $(\emptyset,\emptyset)\models(\emptyset,\emptyset)$.
			We also get $(w,env)\models\Gamma$ and $(w,env)\models(\emptyset,\emptyset)$.



==> sections/Proof/TProof/let.tex <==
\item[\runa{Let}] Here, $e^p=[\mbox{let}\;x\;e_1^{p'}\;e_w^{p''}]^p$, where we have:
			\begin{itemize}
				\item $\Gamma,\Pi\vdash [\mbox{let}\;x\;e_1^{p'}\;e_2^{p''}]^p:T$,
				\item $env\vdash\left\langle [\mbox{let}\;x\;e_1^{p'}\;e_2^{p''}]^p,w,sto,p_3\right\rangle\rightarrow\left\langle v,w',sto',(L,V),p\right\rangle$,
			\end{itemize}
			and that $(w,env)\models T$ and $(w,env)\models\Gamma$.

			To conclude the $[let]$ rule, we need to analyse the premises in the collection semantics and type system.
			In the collection semantics, we have the following:
			\begin{figure}[H]
			\setlength\tabcolsep{8pt}
			\begin{tabular}{l}
				\runa{Let}
				\inference[]
				{env\vdash \left\langle e_1^{p'},sto,w,p \right\rangle \rightarrow \left\langle v',sto'',w'',(L',V'),p' \right\rangle &\\
				env[x\mapsto v]\vdash \left\langle e_2^{p''},sto'',w_3,p' \right\rangle \rightarrow \left\langle v,sto',w',(L,V),p'' \right\rangle}
				{env\vdash \left\langle [\mbox{let}\;x\;e_1^{p'}\;e_2^{p''}]^{p_3},sto,w,p \right\rangle \rightarrow \left\langle v,sto',w',(L,V),p_3 \right\rangle}\\
				Where $w_3=w''[x^{p'}\mapsto(L,V)]$\\[1cm]
			\end{tabular}
			\end{figure}
			And in the type system, we have the following:
			\begin{figure}[H]
			\setlength\tabcolsep{8pt}
			\begin{tabular}{l}
				\runa{Let}
				\inference[]
				{\Gamma;\Pi\vdash e_1^{p'}:T_1 &\\
				\Gamma,x^{p'}:T_1;\Pi\vdash e_2^{p''}:T}
				{\Gamma;\Pi\vdash [\mbox{let}\; x \; e_1^{p'} \; e_2^{p''}]^{p_3}:T}\\[1cm]
			\end{tabular}
			\end{figure}

			In the first premise, if we know that $(w,env)\models T_1$, then from the induction hypothesis, we can immediately get that $\Gamma;\Pi\vdash v':T_1$, $(w'',env)\models T_1$, $(w',env)\models\Gamma$, and $(L',V')\models T_1$.
			Where we also know that an extension of $w$ holds, and $w'$ is an extension of $w$, then to conclude the first premise we need to find out if $(w,env)\models T_1$ holds.
			Here, we know that $\Gamma;\Pi\vdash v':T_1$, and we know that if $x$ occurs in $e_2^{p''}$, then $(w,env)\models T_1$ must hold by the substitution lemma.

			In the second premise, we already know that $(w'',env)\models T$ where we know that $w''$ is an extension of $w$, and thus $w=w''\mid_p$.
			Then for the second premise to hold, we also need to show for $env[x\mapsto v']$.
			If we know that $(w'',env[x\mapsto v'])\models T$, then by our induction hypothesis we can immediately get $\Gamma,x^{p'}:T_1;\Pi\vdash v:T$, $(w',env[x\mapsto v'])\models\Gamma,x^{p'}:T_1$, $(w',env[x\mapsto v'])\models T$, and $(L,V)\models T$.
			Since $env[x\mapsto v']$ is a local extension, and we know the type and dependencies of $v'$, we also know that $(w'',env[x\mapsto v])\models T$, and can be further proven by the use of the substitution lemma.
			From this, the conclusion is follows.


==> sections/Proof/TProof/var.tex <==
\item[\runa{Var}] Here, $e^p=x^p$, where we have:
			\begin{itemize}
				\item $\Gamma,\Pi\vdash x^p:T$, where $\Lambda(x,p)=p''$, $\Gamma(x^{p''})=T'$, and $T=T'\sqcup(\{x^p\},\emptyset)$,
				\item $env\vdash\left\langle x^p,w,sto,p'\right\rangle\rightarrow\left\langle v,w,sto,(L,V\cup\{x^p\}),p\right\rangle$, where $env(x)=v$, $inf_p(x^p,w)=p''$, and $w(x^{p''})=(L,V)$,
			\end{itemize}
			and that $(w,env)\models\Gamma$ and $(w,env)\models T$.

			We can the immediately get that $(w,env)\models T$ and $(w,env)\models \Gamma$.
			From this we can get that $(L,V\cup\{x^p\})\models T$, and then we can conclude that $\Gamma,\Pi\vdash v:T$.

